Invisible Backdoor Attacks Using Data Poisoning in the Frequency Domain

With the broad application of deep neural networks (DNNs), backdoor attacks have gradually attracted attention. Backdoor attacks are insidious, and poisoned models perform well on benign samples and are only triggered when given specific inputs, which cause the neural network to produce incorrect outputs. The state-of-the-art backdoor attack work is implemented by data poisoning, i.e., the attacker injects poisoned samples into the dataset, and the models trained with that dataset are infected with the backdoor. However, most of the triggers used in the current study are fixed patterns patched on a small fraction of an image and are often clearly mislabeled, which is easily detected by humans or defense methods such as Neural Cleanse and SentiNet. Also, it's difficult to be learned by DNNs without mislabeling, as they may ignore small patterns. In this paper, we propose a generalized backdoor attack method based on the frequency domain, which can implement backdoor implantation without mislabeling and accessing the training process. It is invisible to human beings and able to evade the commonly used defense methods. We evaluate our approach in the no-label and clean-label cases on three datasets (CIFAR-10, STL-10, and GTSRB) with two popular scenarios (self-supervised learning and supervised learning). The results show our approach can achieve a high attack success rate (above 90%) on all the tasks without significant performance degradation on main tasks. Also, we evaluate the bypass performance of our approach for different kinds of defenses, including the detection of training data (i.e., Activation Clustering), the preprocessing of inputs (i.e., Filtering), the detection of inputs (i.e., SentiNet), and the detection of models (i.e., Neural Cleanse). The experimental results demonstrate that our approach shows excellent robustness to such defenses.

==> sections/Background.tex <==
\section{Background}
% \subsection{Self-supervised Learning \& Supervised learning}
% \lpz{This subsection may be not necessary, we can only list related work in Section 3.}

% \subsection{Backdoors Attacks in DNNs}
% \yue{introduce clean label backdoor attack, and describe the condition that the attack can succeed} Backdoor attack is a type of attack that meets the following requirements: i) A true result will be predicted on clean data expected as clean models. ii) Once the clean data stamped with a trigger, the model will classify this type of input into a specified/pre-defined label.

\subsection{Spatial Domain and Frequency Domaim}
Spatial domain, also called image space, is a domain we can operate directly on the pixels of the original images. In the spacial domain, RGB and YUV are two commonly used color spaces to record or display color images. Both of them are based upon the perceptual capabilities of human eye. RGB describes a combination of red, green and blue, whereas YUV represents luminance (denoted as "Y" channel) which describes the intensity of light and chrominance (denoted as "U" and "V" channels) which carries the color information. As is discussed in the former work\cite{Podpora2014YUVVR}, YUV color space is more similar to human vision than RGB, and has perceptually better quality, so YUV is becoming more and more widely used in the field of image processing\cite{Xu2020LearningIT}.
% Besides, converting an image to YUV color space gives possibility to process the luminance and chrominance signals independently because a slightly large change of the chrominance signals may pass unnoticed to human beings. The character of YUV helps us to design a more powerful trigger.

Any image in spatial domain can be represented in a frequency domain. The frequency domain provides a new perspective for images processing.
% i.e., an image can be decomposed into a linear superposition of a simple vibration function with different amplitudes, frequencies and phases. 
In the frequency domain, low frequency components correspond to the smooth regions in an image, and high frequency components correspond to edges in an image. 

The spatial domain and the frequency domain can be transformed to each other by Fourier transform. DFT (Discrete Fourier Transform) and DCT (Discrete Cosine Transform) are the most classical transformation methods. DCT is developed from DFT, and has better energy aggregation in frequency domain compared to DFT, so it has been widely used in digital image processing.
% We apply DCT to do the transformation in our experiments, too.

The two-dimensional DCT and IDCT are showed as below:

% \begin{equation}
% \label{DCT}
% F(u,v)=c(u)c(v)\sum_{i=0}^{M-1}\sum_{j=0}^{N-1}f(i,j)\cos{[\frac{(i+0.5)\pi}{M}u]}\cos{[\frac{(j+0.5)\pi}{N}v]}
% \end{equation} 

% \begin{equation}
% \label{IDCT}
% f(i,j)=\sum_{u=0}^{M-1}\sum_{v=0}^{N-1}c(u)c(v)F(u,v)\cos{[\frac{(i+0.5)\pi}{M}u]}\cos{[\frac{(j+0.5)\pi}{N}v]}
% \end{equation} 

\begin{equation}
\label{DCT}
F(u,v)=\sum_{i=0}^{M-1}\sum_{j=0}^{N-1}f(i,j)G(i,j,u,v)
\end{equation} 

\begin{equation}
\label{IDCT}
f(i,j)=\sum_{u=0}^{M-1}\sum_{v=0}^{N-1}F(u,v)G(i,j,u,v)
\end{equation} 

where,

\begin{equation}
\label{IDCT}
G(i,j,u,v)=c(u)c(v)\cos{[\frac{(i+0.5)\pi}{M}u]}\cos{[\frac{(j+0.5)\pi}{N}v]}
\end{equation} 

and

\begin{flalign}
    c(u)=\begin{cases}
    \sqrt{\frac{1}{M}},u=0\\
    \sqrt{\frac{2}{M}},u\ne0
         \end{cases}
    & \ \ \ c(v)=\begin{cases}
    \sqrt{\frac{1}{N}},v=0\\
    \sqrt{\frac{2}{N}},v\ne0
         \end{cases}
\end{flalign}

In the equations above, the DCT transforms an image with size $M \times N$ from the image domain to the frequency domain with the same size, and the IDCT is exactly the opposite.  $F(u,v)$ represents the intensity at the frequency $(u,v)$ in the frequency domain, and $f(i,j)$ represents the pixel value at the position $(i,j)$ in the color space. 

% Figure\ref{} shows an example of an image transformed from the spatial domain to the frequency domain using DCT.

\subsection{Learning in the Frequency Domain}

Current studies have showed that DNN models can perceive information in the frequency domain. \cite{Xu2019TrainingBO, Xu2020FrequencyPF, Luo2021TheoryOT} have demonstrated that a DNN model tends to learn components from low-frequency to high-frequency. \cite{Yin2019AFP, Wang2020HighFrequencyCH} discusses the relation between the robustness and generalization of an DNN model and the frequency properties of training data in the frequency domain. \cite{Gueguen2018FasterNN, Xu2020LearningIT} directly extracts features from the frequency domain to classify images. This may lead to a new domain to perform data poisoning attack.

==> sections/Defense.tex <==
% \section{Defense by Filterring}


